Unmanned Aerial Vehicles: A Survey on Civil Applications and Key Research Challenges

The use of unmanned aerial vehicles (UAVs) is growing rapidly across many civil application domains including real-time monitoring, providing wireless coverage, remote sensing, search and rescue, delivery of goods, security and surveillance, precision agriculture, and civil infrastructure inspection. Smart UAVs are the next big revolution in UAV technology promising to provide new opportunities in different applications, especially in civil infrastructure in terms of reduced risks and lower cost. Civil infrastructure is expected to dominate the more that $45 Billion market value of UAV usage. In this survey, we present UAV civil applications and their challenges. We also discuss current research trends and provide future insights for potential UAV uses. Furthermore, we present the key challenges for UAV civil applications, including: charging challenges, collision avoidance and swarming challenges, and networking and security related challenges. Based on our review of the recent literature, we discuss open research challenges and draw high-level insights on how these challenges might be approached.

==> Table_security.tex <==

\begin{sidewaystable*}[]
\footnotesize
\centering
\caption{\uppercase{The summary of the literature of state-of-the-art attacks and countermeasures for UAV}}
\label{t3}
\begin{tabular}{|l|l|l|l|l|l|l|}
\hline
\multicolumn{1}{|c|}{\textbf{}}   & \multicolumn{1}{c|}{\textbf{Year}} & \multicolumn{1}{c|}{\textbf{Attack Vector}} & \multicolumn{1}{c|}{\textbf{Category}}                                                      & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Proposed\\ Countermeasure\end{tabular}}}                                                          & \multicolumn{1}{c|}{\textbf{Limitations}}                                                                                                                          & \multicolumn{1}{c|}{\textbf{\begin{tabular}[c]{@{}c@{}}Suggested \\ Countermeasures\end{tabular}}}                                                                                                                                                \\ \hline
\cite{javaid2012cyber}          & 2012                               & Communication Links, UAV, GCSs              & C                                                                                           & N/A                                                                                                                                                      & N/A                                                                                                                                                                & N/A                                                                                                                                                                                                                                               \\ \hline
\cite{giray2013anatomy}         & 2013                               & Communication Links                         & \begin{tabular}[c]{@{}l@{}}A: Signal integrity\\  (GPS spoofing)\end{tabular}               & \begin{tabular}[c]{@{}l@{}}1. Cryptography based\\ signal authentication;\\ 2. Multiple receiver design.\end{tabular}                                    & \begin{tabular}[c]{@{}l@{}}1. Lack of details;\\ 2. Require hardware changes \\ (i.e., complexity and cost issue).\end{tabular}                                    & \begin{tabular}[c]{@{}l@{}}1. Strong authentication \\ (e.g., trust platform module,\\  Kerberos, etc.);\\ 2. Signal distortion detection;\\ 3. Direction-of-arrival sensing \\ (i.e.,  transmitter antenna \\ direction detection).\end{tabular} \\ \hline
\cite{javaid2013uavsim}         & 2013                               & Communication Links, UAV, GCSs              & B-1                                                                                         & N/A                                                                                                                                                      & N/A                                                                                                                                                                & N/A                                                                                                                                                                                                                                               \\ \hline
\cite{goppert2014software}      & 2014                               & Communication Links, UAV, GCSs              & C                                                                                           & N/A                                                                                                                                                      & N/A                                                                                                                                                                & N/A                                                                                                                                                                                                                                               \\ \hline
\cite{maxa2015secure}           & 2015                               & Communication Links, UAVs                   & \begin{tabular}[c]{@{}l@{}}A: Routing attack\\ (eavesdropping, DOS, etc.)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}A secure routing protocol\\ and its modeling process.\end{tabular}                                                            & \begin{tabular}[c]{@{}l@{}}Lack of evaluations \\ or security proof.\end{tabular}                                                                                  & \begin{tabular}[c]{@{}l@{}}Perform evaluations under \\ various attack scenarios \\ or provide theoretical \\ security proof.\end{tabular}                                                                                                        \\ \hline
\cite{schumann2015r2u2}         & 2015                               & UAVs                                        & B-2                                                                                         & N/A                                                                                                                                                      & N/A                                                                                                                                                                & N/A                                                                                                                                                                                                                                               \\ \hline
\cite{birnbaum2015unmanned}     & 2015                               & UAVs                                        & B-1                                                                                         & N/A                                                                                                                                                      &                                                                                                                                                                    &                                                                                                                                                                                                                                                   \\ \hline
\cite{muzzi2015using}           & 2015                               & Communication Links, UAVs                   & A: DDoS                                                                                     & \begin{tabular}[c]{@{}l@{}}Botnet platform\\  (as a future work).\end{tabular}                                                                           & \begin{tabular}[c]{@{}l@{}}There is no concrete \\ solution provided.\end{tabular}                                                                                 & \begin{tabular}[c]{@{}l@{}}1. Delivers behavior-based \\ anomaly detection\\  (e.g., packet analysis about \\ its type, rate, volume, \\ source IP, etc.);\\ 2. Enables immediate \\ response to DDoS attacks;\end{tabular}                       \\ \hline
\cite{vattapparamban2016drones} & 2016                               & Communication Links, UAV, GCSs              & C                                                                                           & N/A                                                                                                                                                      & N/A                                                                                                                                                                & N/A                                                                                                                                                                                                                                               \\ \hline
\cite{sedjelmaci2016detect}     & 2016                               & Communication Links, UAV, GCSs              & B-3                                                                                         & N/A                                                                                                                                                      & N/A                                                                                                                                                                & N/A                                                                                                                                                                                                                                               \\ \hline
\cite{davidson2016controlling}  & 2016                               & Communication Links, UAVs                   & \begin{tabular}[c]{@{}l@{}}A: Signal integrity\\  (sensor input spoofing)\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Optical flow analysis\\ (RANSAC algorithm\\ \cite{fischler1981random})\end{tabular}                                         & \begin{tabular}[c]{@{}l@{}}The attack model is too \\ demanding (i.e., it is difficult \\ to perform this attack. ).\end{tabular}                                  & \begin{tabular}[c]{@{}l@{}}1. Strong firewall/authentication \\ schemes to prevent hijacking attacks;\\ 2. Delivers behavior-based \\ anomaly detection.\end{tabular}                                                                             \\ \hline
\cite{mcneely2016detection}     & 2016                               & UAVs                                        & A: UAV hijacking                                                                            & \begin{tabular}[c]{@{}l@{}}Profiling of in-flight\\ statistics.\end{tabular}                                                                             & \begin{tabular}[c]{@{}l@{}}Temporary control instability\\  (e.g., short time decreasing of\\ amplitude) caused by\\ the attacker cannot be detected.\end{tabular} & \begin{tabular}[c]{@{}l@{}}1. Decreasing the detection \\ interval;\\ 2. Strong firewall/authentication \\ schemes to prevent hijacking attacks;\\ 3. Packets analysis of malicious \\ injected commands.\end{tabular}                            \\ \hline
\cite{hagerman2016security}     & 2016                               & N/A                                         & B-2                                                                                         & N/A                                                                                                                                                      & N/A                                                                                                                                                                & N/A                                                                                                                                                                                                                                               \\ \hline
\cite{rodday2016exploring}      & 2016                               & Communication Links                         & \begin{tabular}[c]{@{}l@{}}A: Hijacking \\ (MitM attack)\end{tabular}                       & \begin{tabular}[c]{@{}l@{}}1. XBee 868LP on-board\\ encryption;\\ 2. Dedicated hardware\\ encryption;\\ 3. Application layer \\ encryption.\end{tabular} & No details provided.                                                                                                                                               & \begin{tabular}[c]{@{}l@{}}1. Integrate detection and immediate \\ response mechanisms.\\ 2. Strong authentication \\ (e.g., trust platform module, Kerberos, etc.);\end{tabular}                                                                 \\ \hline
\cite{wang2016authentication}   & 2017                               & Communication Links                         & \begin{tabular}[c]{@{}l@{}}A: Authentication/key\\ management targeted attacks\end{tabular} & \begin{tabular}[c]{@{}l@{}}A set of modified \\ authentication and key\\ management protocols.\end{tabular}                                              & \begin{tabular}[c]{@{}l@{}}Lack of evaluations \\ or security proof.\end{tabular}                                                                                  & \begin{tabular}[c]{@{}l@{}}Perform evaluations under \\ various attack scenarios \\ or provide theoretical \\ security proof.\end{tabular}                                                                                                        \\ \hline
\cite{podhradsky2017improving}  & 2017                               & Communication Links, GCS, UAV               & C                                                                                           & N/A                                                                                                                                                      & N/A                                                                                                                                                                & N/A                                                                                                                                                                                                                                               \\ \hline
\end{tabular}
\end{sidewaystable*}

==> Table_surveillance.tex <==
\begin{table*}[]
\normalsize
\centering
\caption{\uppercase{Summary of UAV applications for security surveillance}}
\label{t1}
\begin{tabular}{|l|l|c|c|}
\hline
\multicolumn{1}{|c|}{\textbf{Surveillance}} & \multicolumn{1}{c|}{\textbf{Year}} & \textbf{Research Focus}                                                                                                           & \textbf{Category}            \\ \hline
\cite{kingston2008decentralized}                                                & 2008                               & UAVs cooperative perimeter surveillance                                                                                           & Multi-UAV cooperation        \\ \hline
\cite{haddal2010homeland}                                                & 2010                               & UAV with border surveillance                                                                                                      & Homeland security concerns   \\ \hline
\cite{maza2011experimental}                                                & 2011                               & \begin{tabular}[c]{@{}c@{}}Multi-UAV coordination for disaster management \\ and civil security applications\end{tabular}         & Multi-UAV cooperation       \\ \hline
\cite{wall2011surveillance}                                                & 2011                               & Concerns of UAVs in battle filed                                                                                                  & Military concerns            \\ \hline
\cite{birk2011safety}                                                & 2011                               & \begin{tabular}[c]{@{}c@{}}UAV system filed tests with improved \\ photo mapping algorithm\end{tabular}                           & Algorithm improvement        \\ \hline
\cite{finn2012unmanned}                                                & 2012                               & \begin{tabular}[c]{@{}c@{}}UAV surveillance in civil applications impacts \\ upon privacy and other civil liberties\end{tabular} & Privacy and civil liberties \\ \hline
\cite{wada2015surveillance}                                                & 2015                               & A small UAV system with related technologies                                                                                      & Product introduction         \\ \hline
\cite{motlagh2017uav}                                                & 2017                               & UAV-based IoT platform for crowd surveillance                                                                                     & New use case                 \\ \hline
\end{tabular}
\end{table*}
